ALERT: Adapting Language Models to Reasoning Tasks

Current large language models can perform reasonably well on complex tasks that require step-by-step reasoning with few-shot learning. Are these models applying reasoning skills they have learnt during pre-training and reason outside of their training context, or are they simply memorizing their training corpus at finer granularity and have learnt to better understand their context? To tease apart these possibilities, we introduce ALERT, a benchmark and suite of analyses for assessing language models' reasoning ability comparing pre-trained and finetuned models on complex tasks that require reasoning skills to solve. ALERT provides a test bed to asses any language model on fine-grained reasoning skills, which spans over 20 datasets and covers 10 different reasoning skills. We leverage ALERT to further investigate the role of finetuning. With extensive empirical analysis we find that language models learn more reasoning skills such as textual entailment, abductive reasoning, and analogical reasoning during finetuning stage compared to pretraining state. We also find that when language models are finetuned they tend to overfit to the prompt template, which hurts the robustness of models causing generalization problems.

==> sections/checklist.tex <==
\subsection{Did you discuss the \textit{limitations} of your work?}
If you answer {\bf Yes}, provide the section number; if you answer {\bf No}, provide a justification. \\[0.3cm]
\begin{Form}
\begin{tabular}{l}
    \cm{mainClaims}{Yes,No,N/A}{}\\[0.2cm]
    \tf[0.85]{mainClaimsJustification}{}
\end{tabular}
\end{Form} \\[0.3cm]

\subsection{Did you discuss any potential \textit{risks} of your work?}
If you answer {\bf Yes}, provide the section number; if you answer {\bf No}, provide a justification. \\[0.3cm]
\begin{Form}
\begin{tabular}{l}
    \cm{risks}{Yes,No,N/A}{}\\[0.2cm]
    \tf[0.85]{risksJustification}{}
\end{tabular}
\end{Form}

\subsection{Do the abstract and introduction summarize the paper’s main claims?}
If you answer {\bf Yes}, provide the section number; if you answer {\bf No}, provide a justification. \\[0.3cm]
\begin{Form}
\begin{tabular}{l}
    \cm{abstractIntro}{Yes,No,N/A}{}\\[0.2cm]
    \tf[0.85]{abstractIntroJustification}{}
\end{tabular}
\end{Form}

\section{Did you use or create \textit{scientific artifacts}?}
If you answer {\bf Yes}, provide the section number; if you answer {\bf No}, you can skip the rest of this section. \\[0.3cm]
\begin{Form}
\begin{tabular}{l}
\cm{createArtifacts}{Yes,No}{}\\[0.2cm]
\end{tabular}
\end{Form}

If yes:
\subsection{Did you cite the creators of artifacts you used?}
If you answer {\bf Yes}, provide the section number; if you answer {\bf No}, provide a justification. \\[0.3cm]
\begin{Form}
   \begin{tabular}{l}
    \cm{citeCreators}{Yes,No,N/A}{}\\[0.2cm]
    \tf{citeCreatorsJustification}{}
\end{tabular}
\end{Form} \\[0.3cm]

\subsection{Did you discuss the \textit{license or terms} for use and/or distribution of any artifacts?}
If you answer {\bf Yes}, provide the section number; if you answer {\bf No}, provide a justification. \\[0.3cm]
\begin{Form}
   \begin{tabular}{l}
    \cm{legalGrounds}{Yes,No,N/A}{}\\[0.2cm]
    \tf{legalGroundsJustification}{}
\end{tabular}
\end{Form} \\[0.3cm]

\subsection{Did you discuss if your use of existing artifact(s) was consistent with their \textit{intended use}, provided that it was specified? For the artifacts you create, do you specify intended use and whether that is compatible with the original access conditions (in particular, derivatives of data accessed for research purposes should not be used outside of research contexts)?}
If you answer {\bf Yes}, provide the section number; if you answer {\bf No}, provide a justification. \\[0.3cm]
\begin{Form}
   \begin{tabular}{l}
    \cm{intendedUse}{Yes,No,N/A}{}\\[0.2cm]
    \tf{intendedUseJustification}{}
\end{tabular}
\end{Form} \\[0.3cm]

\subsection{Did you discuss the steps taken to check whether the data that was collected/used contains any \textit{information that names or uniquely identifies individual people} or \textit{offensive content}, and the steps taken to protect / anonymize it?}
If you answer {\bf Yes}, provide the section number; if you answer {\bf No}, provide a justification. \\[0.3cm]
\begin{Form}
\begin{tabular}{l}
    \cm{personallyIdentifiableInformationOrOffensiveContent}{Yes,No,N/A}{}\\[0.2cm]
    \tf{personallyIdentifiableInformationOrOffensiveContentJustification}{}
\end{tabular}
\end{Form} \\[0.3cm]

\subsection{Did you provide documentation of the artifacts, e.g., coverage of domains, languages, and linguistic phenomena, demographic groups represented, etc.?}
If you answer {\bf Yes}, provide the section number; if you answer {\bf No}, provide a justification. \\[0.3cm]
\begin{Form}
\begin{tabular}{l}
    \cm{documentation}{Yes,No,N/A}{}\\[0.2cm]
    \tf{documentationJustification}{}
\end{tabular}
\end{Form} \\[0.3cm]

\subsection{Did you report relevant statistics like the number of examples, details of train/test/dev splits, etc. for the data that you used/created?}
If you answer {\bf Yes}, provide the section number; if you answer {\bf No}, provide a justification. \\[0.3cm]
\begin{Form}
\begin{tabular}{l}
    \cm{relevantStatistics}{Yes,No,N/A}{}\\[0.2cm]
    \tf{relevantStatisticsJustification}{}
\end{tabular}
\end{Form} \\[0.3cm]

\section{Did you run \textit{computational experiments}?} 
If you answer {\bf Yes}, provide the section number; if you answer {\bf No}, you can skip the rest of this section. \\[0.3cm]
\begin{Form}
\begin{tabular}{l}
    \cm{computationalExperiments}{Yes,No}{}
\end{tabular}
\end{Form}

If yes:
\subsection{Did you report the \textit{number of parameters} in the models used, the \textit{total computational budget} (e.g., GPU hours), and \textit{computing infrastructure} used?}
If you answer {\bf Yes}, provide the section number; if you answer {\bf No}, provide a justification. \\[0.3cm]
\begin{Form}
\begin{tabular}{l}
    \cm{reportReproducibility}{Yes,No,N/A}{}\\[0.2cm]
    \tf{reportReproducibilityJustification}{}
\end{tabular}
\end{Form} \\[0.3cm]

\subsection{Did you discuss the experimental setup, including \textit{hyperparameter search} and \textit{best-found hyperparameter} values?}
If you answer {\bf Yes}, provide the section number; if you answer {\bf No}, provide a justification. \\[0.3cm]
\begin{Form}
\begin{tabular}{l}
    \cm{bestFoundHyperparameter}{Yes,No,N/A}{}\\[0.2cm]
    \tf{bestFoundHyperparameterJustification}{}
\end{tabular}
\end{Form} \\[0.3cm]

\subsection{Did you report \textit{descriptive statistics} about your results (e.g., error bars around results, summary statistics from sets of experiments), and is it transparent whether you are reporting the max, mean, etc. or just a single run?}
If you answer {\bf Yes}, provide the section number; if you answer {\bf No}, provide a justification. \\[0.3cm]
\begin{Form}
\begin{tabular}{l}
    \cm{descriptiveStatistics}{Yes,No,N/A}{}\\[0.2cm]
    \tf{descriptiveStatisticsJustification}{}
\end{tabular}
\end{Form} \\[0.3cm]

\subsection{If you used existing packages (e.g., for preprocessing, for normalization, or for evaluation), did you report the implementation, model, and parameter settings used (e.g., NLTK, Spacy, ROUGE, etc.)?}
If you answer {\bf Yes}, provide the section number; if you answer {\bf No}, provide a justification. \\[0.3cm]
\begin{Form}
\begin{tabular}{l}
    \cm{existingPackages}{Yes,No,N/A}{}\\[0.2cm]
    \tf{existingPackagesJustification}{}
\end{tabular}
\end{Form} \\[0.3cm]

\section{Did you use \textit{human annotators} (e.g., crowdworkers) or \textit{research with human subjects}?}  If you answer {\bf Yes}, provide the section number; if you answer {\bf No}, you can skip the rest of this section. \\[0.3cm]
\begin{Form}
\begin{tabular}{l}
    \cm{hummanAnnotators}{Yes,No}{}\\
\end{tabular}
\end{Form}

If yes:
\subsection{Did you report the full text of instructions given to participants, including e.g., screenshots, disclaimers of any risks to participants or annotators, etc.?}
If you answer {\bf Yes}, provide the section number; if you answer {\bf No}, provide a justification. \\[0.3cm]
\begin{Form}
\begin{tabular}{l}
    \cm{fullTextInstructions}{Yes,No,N/A}{}\\[0.2cm]
    \tf{fullTextInstructionsJustification}{}
\end{tabular}
\end{Form} \\[0.3cm]

\subsection{Did you report information about how you recruited (e.g., crowdsourcing platform, students) and paid participants, and discuss if such \textit{payment is adequate} given the participants’ demographic (e.g., country of residence)?}
If you answer {\bf Yes}, provide the section number; if you answer {\bf No}, provide a justification. \\[0.3cm]
\begin{Form}
\begin{tabular}{l}
    \cm{payment}{Yes,No,N/A}{}\\[0.2cm]
    \tf{paymentJustification}{}
\end{tabular}
\end{Form} \\[0.3cm]

\subsection{Did you discuss whether and how \textit{consent} was obtained from people whose data you're using/curating (e.g., did your instructions explain how the data would be used)?}
If you answer {\bf Yes}, provide the section number; if you answer {\bf No}, provide a justification. \\[0.3cm]
\begin{Form}
\begin{tabular}{l}
    \cm{consent}{Yes,No,N/A}{}\\[0.2cm]
    \tf{consentJustification}{}
\end{tabular}
\end{Form} \\[0.3cm]

\subsection{Was the data collection protocol \textit{approved (or determined exempt)} by an ethics review board?}
If you answer {\bf Yes}, provide the section number; if you answer {\bf No}, provide a justification. \\[0.3cm]
\begin{Form}
\begin{tabular}{l}
    \cm{ethicsAmountSpent}{Yes,No,N/A}{}\\[0.2cm]
    \tf{ethicsAmountSpentJustification}{}
\end{tabular}
\end{Form} \\[0.3cm]

\subsection{Did you report the basic demographic and geographic characteristics of the \textit{annotator} population that is the source of the data?}
If you answer {\bf Yes}, provide the section number; if you answer {\bf No}, provide a justification. \\[0.3cm]
\begin{Form}
\begin{tabular}{l}
    \cm{annotator}{Yes,No,N/A}{}\\[0.2cm]
    \tf{annotatorJustification}{}
\end{tabular}
\end{Form} \\[0.3cm]



==> tables/table-roscoe-062.tex <==
\begin{table*}[bht]
\begin{center}
\scalebox{0.85}
    {
 \begin{tabular}{lcccccc}
    \toprule
  & OPT 1.3B & OPT-FT 1.3B & OPT-CoT 1.3B & OPT 13B & OPT-FT 13B & OPT-CoT 13B \\
\midrule
\multicolumn{7}{l}{\texttt{ROSCOE-SA}} \\
\ \ \ \ \ Faithfulness-Step & \textbf{0.822} & 0.761 & 0.773 & 0.797 & 0.770 & \underline{0.799} \\
\ \ \ \ \ Faithfulness-Token & 0.916 & 0.915 & 0.912 & \underline{0.928} & 0.927 & \textbf{0.933} \\
\ \ \ \ \ Info-Step & \textbf{0.819} & 0.759 & 0.773 & 0.796 & 0.766 & \underline{0.800} \\
\ \ \ \ \ Repetition-Token & 0.874 & \underline{0.987} & 0.875 & 0.882 & \textbf{1.000} & 0.824 \\
\multicolumn{7}{l}{\texttt{ROSCOE-SS}} \\
\ \ \ \ \ Info-Chain & \textbf{0.907} & 0.879 & 0.885 & 0.895 & 0.883 & \underline{0.896} \\
\ \ \ \ \ Repetition-Step & 0.876 & \underline{0.987} & 0.883 & 0.884 & \textbf{1.000} & 0.834 \\
\multicolumn{7}{l}{\texttt{ROSCOE-LI}} \\
\ \ \ \ \ Source Consistency & 0.712 & 0.736 & 0.761 & 0.763 & \textbf{0.860} & \underline{0.825} \\
\ \ \ \ \ Self-Consistency & 0.942 & \underline{0.992} & 0.945 & 0.952 & \textbf{0.996} & 0.931 \\
\multicolumn{7}{l}{\texttt{ROSCOE-LS}} \\
\ \ \ \ \ Perplexity-Step & \textbf{0.125} & \underline{0.037} & \textbf{0.125} & 0.035 & 0.036 & \underline{0.037} \\
\ \ \ \ \ Perplexity-Chain & \textbf{0.127} & 0.037 & \underline{0.126} & 0.037 & 0.036 & 0.040 \\
\ \ \ \ \ Grammar & 0.650 & \textbf{0.674} & \underline{0.665} & 0.546 & 0.595 & 0.576 \\
    \bottomrule
    \end{tabular}%
    }
	\end{center}
  \caption{\footnotesize \texttt{ROSCOE} evaluation results, template 062 (\textit{??}). Each metric is bounded within $[0, 1]$, where $1$ indicates the perfect score and $0$ corresponds to failure. Values corresponding to the best performing model are \textbf{bolded}, second best are \underline{underscored}.}
\label{tab:roscoe-062}
\end{table*}

==> tables/table-roscoe-080.tex <==
\begin{table*}[bht]
\begin{center}
\scalebox{0.85}
    {
 \begin{tabular}{lcccccc}
    \toprule
  & OPT 1.3B & OPT-FT 1.3B & OPT-CoT 1.3B & OPT 13B & OPT-FT 13B & OPT-CoT 13B \\
\midrule
\multicolumn{7}{l}{\texttt{ROSCOE-SA}} \\
\ \ \ \ \ Faithfulness-Step & 0.856 & \textbf{0.868} & 0.863 & 0.859 & \underline{0.867} & 0.853 \\
\ \ \ \ \ Faithfulness-Token & \underline{0.932} & \underline{0.932} & \textbf{0.935} & \underline{0.932} & \underline{0.932} & \underline{0.932} \\
\ \ \ \ \ Info-Step & 0.870 & 0.867 & \textbf{0.875} & \underline{0.874} & 0.873 & 0.861 \\
\ \ \ \ \ Repetition-Token & 0.242 & \textbf{0.833} & 0.287 & 0.197 & 0.370 & \underline{0.401} \\
\multicolumn{7}{l}{\texttt{ROSCOE-SS}} \\
\ \ \ \ \ Info-Chain & 0.928 & \textbf{0.933} & 0.925 & \underline{0.931} & 0.929 & 0.918 \\
\ \ \ \ \ Repetition-Step & 0.254 & \textbf{0.836} & 0.298 & 0.205 & 0.378 & \underline{0.409} \\
\multicolumn{7}{l}{\texttt{ROSCOE-LI}} \\
\ \ \ \ \ Source Consistency & 0.750 & 0.823 & 0.705 & \underline{0.850} & \textbf{0.907} & 0.843 \\
\ \ \ \ \ Self-Consistency & 0.759 & \textbf{0.967} & 0.809 & 0.817 & \underline{0.953} & 0.913 \\
\multicolumn{7}{l}{\texttt{ROSCOE-LS}} \\
\ \ \ \ \ Perplexity-Step & 0.008 & 0.006 & 0.007 & \underline{0.010} & 0.008 & \textbf{0.011} \\
\ \ \ \ \ Perplexity-Chain & 0.018 & 0.008 & 0.013 & \textbf{0.021} & 0.013 & \underline{0.020} \\
\ \ \ \ \ Grammar & 0.714 & \underline{0.771} & 0.643 & 0.733 & \textbf{0.779} & 0.678 \\
    \bottomrule
    \end{tabular}%
    }
	\end{center}
  \caption{\footnotesize \texttt{ROSCOE} evaluation results, template 080 (\textit{piqa answer generation}). Each metric is bounded within $[0, 1]$, where $1$ indicates the perfect score and $0$ corresponds to failure. Values corresponding to the best performing model are \textbf{bolded}, second best are \underline{underscored}.}
\label{tab:roscoe-080}
\end{table*}

==> tables/table-roscoe-083.tex <==
\begin{table*}[bht]
\begin{center}
\scalebox{0.85}
    {
 \begin{tabular}{lcccccc}
    \toprule
  & OPT 1.3B & OPT-FT 1.3B & OPT-CoT 1.3B & OPT 13B & OPT-FT 13B & OPT-CoT 13B \\
\midrule
\multicolumn{7}{l}{\texttt{ROSCOE-SA}} \\
\ \ \ \ \ Faithfulness-Step & 0.889 & 0.886 & 0.891 & 0.891 & \underline{0.905} & \textbf{0.915} \\
\ \ \ \ \ Faithfulness-Token & \underline{0.947} & 0.945 & \textbf{0.948} & 0.946 & 0.943 & \textbf{0.948} \\
\ \ \ \ \ Info-Step & 0.885 & 0.871 & 0.879 & 0.886 & \underline{0.888} & \textbf{0.901} \\
\ \ \ \ \ Repetition-Token & 0.265 & 0.401 & \textbf{0.532} & 0.272 & \underline{0.410} & 0.338 \\
\multicolumn{7}{l}{\texttt{ROSCOE-SS}} \\
\ \ \ \ \ Info-Chain & \textbf{0.941} & 0.934 & 0.931 & \textbf{0.941} & \underline{0.936} & 0.935 \\
\ \ \ \ \ Repetition-Step & 0.260 &\underline{0.417} & \textbf{0.535} & 0.266 & 0.400 & 0.330 \\
\multicolumn{7}{l}{\texttt{ROSCOE-LI}} \\
\ \ \ \ \ Source Consistency & 0.004 & 0.013 & 0.035 & 0.005 & 0.015 & 0.024 \\
\ \ \ \ \ Self-Consistency & 0.412 & 0.539 & 0.575 & 0.423 & 0.599 & 0.546 \\
\multicolumn{7}{l}{\texttt{ROSCOE-LS}} \\
\ \ \ \ \ Perplexity-Step & 0.002 & 0.001 & 0.002 & 0.003 & 0.002 & 0.002 \\
\ \ \ \ \ Perplexity-Chain & 0.018 & 0.004 & 0.014 & 0.019 & 0.008 & 0.014 \\
\ \ \ \ \ Grammar & 0.751 & 0.717 & 0.640 & 0.757 & 0.652 & 0.669 \\
    \bottomrule
    \end{tabular}%
    }
	\end{center}
  \caption{\footnotesize \texttt{ROSCOE} evaluation results, template 083 (\textit{??}). Each metric is bounded within $[0, 1]$, where $1$ indicates the perfect score and $0$ corresponds to failure. Values corresponding to the best performing model are \textbf{bolded}, second best are \underline{underscored}.}
\label{tab:roscoe-083}
\end{table*}

==> tables/table-roscoe-detailed-long.tex <==
\begin{table*}[bht]
\vspace{-10pt}
\begin{center}
\scalebox{0.85}
    {
 \begin{tabular}{lcccccc}
    \toprule
  & OPT 1.3B & OPT-FT 1.3B & OPT-CoT 1.3B & OPT 13B & OPT-FT 13B & OPT-CoT 13B \\
\midrule
\multicolumn{7}{l}{\texttt{ROSCOE-SA}} \\
\ \ \ \ \ Faithfulness-Step & 0.858 & \textbf{0.875} & 0.866 & 0.862 & 0.865 & \underline{0.869} \\
\ \ \ \ \ Faithfulness-Token & 0.940 & \textbf{0.947} & \underline{0.946} & 0.942 & 0.941 & \textbf{0.947} \\
\ \ \ \ \ Info-Step & 0.863 & 0.871 & \underline{0.872} & 0.867 & 0.867 & \textbf{0.873} \\
\ \ \ \ \ Repetition-Token & 0.053 & \underline{0.056} & 0.047 & 0.052 & \textbf{0.057} & 0.048 \\
\multicolumn{7}{l}{\texttt{ROSCOE-SS}} \\
\ \ \ \ \ Info-Chain & 0.925 & 0.927 & 0.924 & 0.932 & 0.928 & 0.928 \\
\ \ \ \ \ Repetition-Step & 0.074 & 0.079 & 0.076 & 0.072 & 0.079 & 0.075 \\
\multicolumn{7}{l}{\texttt{ROSCOE-LI}} \\
\ \ \ \ \ Source Consistency & 0.437 & 0.433 & 0.439 & 0.479 & 0.498 & 0.490 \\
\ \ \ \ \ Self-Consistency & 0.628 & 0.685 & 0.595 & 0.696 & 0.719 & 0.718 \\
\multicolumn{7}{l}{\texttt{ROSCOE-LS}} \\
\ \ \ \ \ Perplexity-Step & 0.008 & 0.006 & 0.007 & 0.008 & 0.006 & 0.008 \\
\ \ \ \ \ Perplexity-Chain & 0.026 & 0.018 & 0.030 & 0.023 & 0.020 & 0.023 \\
\ \ \ \ \ Grammar & 0.749 & 0.785 & 0.745 & 0.728 & 0.701 & 0.721 \\
    \bottomrule
\end{tabular}
}
\end{center}
\caption{\footnotesize \texttt{ROSCOE} evaluation results averaged across templates for chains with more than 1 step. Each metric is bounded within $[0, 1]$, where $1$ indicates the perfect score and $0$ corresponds to failure. Values corresponding to the best performing model are \textbf{bolded}, second best are \underline{underscored}.}
\label{tab:roscoe-detailed-long}
\end{table*}

